Flexible SVBRDF Capture with a Multi-Image Deep Network

Empowered by deep learning, recent methods for material capture can estimate a spatially-varying reflectance from a single photograph. Such lightweight capture is in stark contrast with the tens or hundreds of pictures required by traditional optimization-based approaches. However, a single image is often simply not enough to observe the rich appearance of real-world materials. We present a deep-learning method capable of estimating material appearance from a variable number of uncalibrated and unordered pictures captured with a handheld camera and flash. Thanks to an order-independent fusing layer, this architecture extracts the most useful information from each picture, while benefiting from strong priors learned from data. The method can handle both view and light direction variation without calibration. We show how our method improves its prediction with the number of input pictures, and reaches high quality reconstructions with as little as 1 to 10 images -- a sweet spot between existing single-image and complex multi-image approaches.

==> 3_overview.tex <==
\section{Overview}
\label{methodOverview}

\AB{I felt that the overview was actually providing too many details, leaving the technical section quite empty or repetitive. I shortened it and moved the relevant material to subsequent sections.}

Figure~\ref{fig:overview} illustrates the main components of our method. Our overall goal is to estimate the spatially-varying bi-directional reflectance distribution function (SVBRDF) of a flat material sample given a few pictures of that sample. We adopt a parametric representation of the SVBRDF in the form of four maps representing the per-pixel surface normal and diffuse albedo, specular albedo and specular roughness of a Cook-Torrance~\shortcite{Cook82} BRDF model.

Our method relies on deep learning to infer material parameters from pictures. A significant part of our approach is thus devoted to generating data with ground truth parameters to supervise the training.
We implemented this data generation as an online system, which synthesizes a unique SVBRDF and renders it under the target viewing and lighting conditions at each training iteration (Section~\ref{} and Figure~\ref{fig:overview}a).

Once generated, the unique set of training images is fed to our deep network, which is composed of several copies of the same encoder-decoder that process each of the images in parallel (Section~\ref{} and Figure~\ref{fig:overview}b). The output feature maps of these parallel tracks are then fused before being processed by a series of convolutions and non-linearities to produce the output SVBRDF. 

Thanks to its flexible data generation and network architecture, our method can handle a variety of multi-image capture scenarios. In particular, we compare three instances of our approach (Section~\ref{}), each providing different trade-offs. In all cases, our evaluation shows that the quality of prediction improves as more images are provided to our method, resulting in a significant gain over single-image methods with as little as $5$ to $10$ images (Section~\ref{}) \AB{update those numbers once we have the evaluation}\MA{In general I'd suspect that the greatest improvement is achieved with the second photo, and then it tapers off fairly quickly. But we'll see}.\GD{Maybe add: In addition, the flexibility of our method allows exploration of several different configurations, allowing us to identify good strategies for different capture and rendering requirements.}

%Our method aims at bridging the gap between one-picture acquisition methods and complex acquisition setups. Using only one flash picture, many effects are almost impossible to observe. Furthermore, details are lost and normals look flatter than they are because most shadows are squashed when using a frontal flash. At the other extreme, complex acquisition rigs allow for high precision but are expensive, requiring long measurement times and extensive calibration.

%We train a neural network to take an arbitrary number of pictures of a material with different lighting conditions as input and extract a SVBRDF representation (diffuse, specular, roughness, normal \DEL{and anisotropy}).

%To allow for arbitrary number and order of inputs, we first use a copy of a single-image acquisition network as defined by Deschaintre et al.~\shortcite{Deschaintre18} for each input. These evaluations are forwarded to a max pooling layer to aggregate the most relevant features. Finally, a CNN processes the aggregated information to output the SVBRDFs parameter maps.

%We use Deschaintre et al.~\shortcite{Deschaintre18} material set for the training. Instead of using a predefined amount of renderings, we generate the training data on the fly. Using a simple renderer implemented in the network code, we generate renderings with different materials, view and light conditions and augmentation parameters dynamically. This makes our method very easy to adapt to many acquisition processes

%We demonstrate the flexibility of our method by training it for three different capture scenarios: fixed camera and controlled lighting, hand-held camera and light, and hand-held camera and light augmented with a paper frame. \AB{Clarify once we know which scenarios we will implement.}


%We finally combine multiple losses with different weights. A rendering loss, comparing multiple light and view conditions renderings of the outputs and ground truths, both with a perceptual metric and L1 distance. We also use a L1 distance directly on the material parameter maps, learning to decorrelate maps from the input albedo/normal appearance. 

%In Section \ref{sec:input_variation_impact} we discuss the input variation impact, we then describe in more detail our architecture in Section \ref{sec:architecture}, our dataset in Section \ref{sec:dataset} and our training environment in Section\ref{sec:training}. We finally thoroughly evaluate and compare our method both quantitatively and qualitatively in Section \ref{sec:Evaluation}.



==> 4_input_variation_impact.tex <==
\section{Impact of input variation}
\label{sec:input_variation_impact}
\subsection{Precision of acquisition}
%Discuss the impact we expect and how we use different light and view from real life images (reprojection, no highlight problem, ... ?)
Lightweight acquisition methods often focus on a single picture, trying to extract as much information as possible despite the ill-posedness of the problem \cite{Li18}\cite{Deschaintre18}\cite{Li17}.
A single flash-picture is convenient in terms of acquisition and gives information about the specular reflectivity of a material, but fails to capture important effects.
Using multiple inputs we aim at reducing several of these shortcomings. 

Both Li et al.~\shortcite{Li18} and Deschaintre et al.~\shortcite{Deschaintre18} suffer from  the loss of information in the material picture where the flash causes over-exposure. Despite effort in both methods to fill-in the missing information, artefacts are still visible in most specular materials. Providing more images directly provides the network with valuable information, allowing to fill-in these missing parts. This effect is visible in fig.\ref{fig:overExposureFillIn}
\begin{figure}[!t]
\includegraphics[width=\linewidth]{img/temp_figure}
\caption{Show renderings of a single material inferred from 1, 2, 3, ... pictures showing that the highlight quickly fades away}
\label{fig:overExposureFillIn}
\end{figure}

Using a fronto-parallel flash-picture setup reduces the shadowing cues available for the network to fully retrieve normals. Adding side-lit pictures of the material provides more information about the shadowing effect created by strong normals, as shown in fig.\ref{fig:normalSquash}


\begin{figure}[!t]
\includegraphics[width=\linewidth]{img/temp_figure}
\caption{Show renderings of a single material inferred from 1, 2, 3, ... pictures with relevant angles showing strong improvement of the normals}
\label{fig:normalSquash}
\end{figure}

Another limitation of single flash-picture methods, is that the specular highlight will often be visible on one material of the whole SVBRDF. This will allow the method to retrieve plausible parameters for this material, but will lack information for any other material in the picture. Providing more pictures gives a chance to the network to get the missing information about all the materials in the pictures, as shown in Fig.\ref{fig:multiMaterialSpecu} 

Solving these limitations reduces the amount of post-processing required to achieve production quality.

\begin{figure}[!t]
\includegraphics[width=\linewidth]{img/temp_figure}
\caption{Show renderings of a single SVBRDF inferred from 1, 2, 3, ... pictures with multiple materials with very different parameters}
\label{fig:multiMaterialSpecu}
\end{figure}

Finally some important effects such as anisotropy are not treated in single picture methods. With more information available, we are able to add parameters to the outputs, providing -on top of specular and diffuse albedos, specularity and roughness- an anisotropy map, see \ref{fig:anisotropicMats}.

\begin{figure}[!t]
\includegraphics[width=\linewidth]{img/temp_figure}
\caption{Show renderings of an anisotropic material with and without anisotropy in the rendering}
\label{fig:anisotropicMats}
\end{figure}

%Talk about what multiple viewpoint can bring (better understanding of material's effects, possibility to represent fresnel/specularity more accurately.

\subsection{Convenience of acquisition}

Most methods require either a specific number of inputs with different conditions \cite{Aittala15} or specific light/view angles \cite{Riviere17}. Depending on how the input pictures are acquired and the available hardware, these two conditions can be hard to meet and are restrictive.

For example, online resources can provide a few pictures of a single material, but it is very unlikely that the desired number, conditions and angles are exactly matched.
Even if the material is physically available, taking specific light/view angles can require careful calibration and specific hardware.

We design our method with acquisition convenience as a priority. We are able to infer a material from just one image, and we improve the result quality for every additional input. 
We therefore give the user the flexibility to use our method regardless of the amount of information he has and to provide more information if he estimates that better quality can be achieved.  

%\subsection{Convenience of use}
%INCLUDE THE ARGUMENT IN THE QUALITY
%One picture methods are very convenient in terms of acquisition but suffer from artefacts around the over-exposed areas. These are woven in the results and hard to isolate through post treatment, making these results difficult to use for artists.
%By offering the possibility to remove these artefacts and improve the results with very little cost in convenience

%The other problem is that is some cases you may not be able to access as many picture as you would like, or they are not precisely at the right angles The user has to precisely align the input pictures, and 


% Talk about the difficulty in acquisition (moving light and viewpoint together/independently, if the viewpoint is very steep, we have to strongly correct the picture, how do we detect the interesting material's borders ? The noise introduced by this correction, ??

%Discuss how we imagine the acquisition setup - explain that the option of using N picture can be easily calibrated. On the opposite having a random amount of picture requires specific treatment by a network if we don't want to have to train N different networks (and the weights coming along).
%We want to keep the acquisition process as casual as possible, and show that for each picture you manage to add on top of your set of existing picture, you improve quality.
%We of course have a full section on evaluation but here is a quick glance at a graph of how the quality evolves given different number of inputs
%Preface that we will have a full evaluation on how more pictures is interesting (depending on how much you should vary the pictures, maybe base on the papers trying to find the optimal amount of pictures/angles ?). Be careful about the forward reference though...

%Our method takes an arbitrary amount of pictures as input. 

==> figures/Synth5Improvement/synth5improvement.tex <==
\begin{figure*}[!t]
\begin{tabular} {ccccccccc}
  & \vspace{0.5mm} \small{Inputs}  &  \vspace{0.5mm} \small{Renderings} &  \vspace{0.5mm} \small{Environment lit} & \vspace{0.5mm} \small{Normal}  & \vspace{0.5mm} \small{Diffuse albedo}  & \vspace{0.5mm} \small{Roughness}  & \vspace{0.5mm} \small{Specular albedo}  &   \\
\begin{sideways} \hspace{-5mm} \small{1 input} \end{sideways} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/28_37_leather_tiles_4-inputs-0-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/slentedRenderings/28_37_leather_tiles_4_4-outputs-_relight.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/envRenderings/env_ennis/28_37_leather_tiles_4_outputs-rerendering.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/28_37_leather_tiles_4-outputs_gammad-0-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/28_37_leather_tiles_4-outputs_gammad-1-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/28_37_leather_tiles_4-outputs_gammad-2-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/28_37_leather_tiles_4-outputs_gammad-3-.png} & \vspace{3mm} \\
\begin{sideways} \hspace{-5mm} \small{2 inputs} \end{sideways} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/1/images/28_37_leather_tiles_4-inputs-1-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/1/slentedRenderings/28_37_leather_tiles_4_4-outputs-_relight.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/1/envRenderings/env_ennis/28_37_leather_tiles_4_outputs-rerendering.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/1/images/28_37_leather_tiles_4-outputs_gammad-0-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/1/images/28_37_leather_tiles_4-outputs_gammad-1-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/1/images/28_37_leather_tiles_4-outputs_gammad-2-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/1/images/28_37_leather_tiles_4-outputs_gammad-3-.png} & \vspace{3mm} \\
\begin{sideways} \hspace{-5mm} \small{3 inputs} \end{sideways} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/images/28_37_leather_tiles_4-inputs-2-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/slentedRenderings/28_37_leather_tiles_4_4-outputs-_relight.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/envRenderings/env_ennis/28_37_leather_tiles_4_outputs-rerendering.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/images/28_37_leather_tiles_4-outputs_gammad-0-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/images/28_37_leather_tiles_4-outputs_gammad-1-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/images/28_37_leather_tiles_4-outputs_gammad-2-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/images/28_37_leather_tiles_4-outputs_gammad-3-.png} & \vspace{3mm} \\
\begin{sideways} \hspace{-5mm} \small{5 inputs} \end{sideways} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/4/images/28_37_leather_tiles_4-inputs-4-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/4/slentedRenderings/28_37_leather_tiles_4_4-outputs-_relight.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/4/envRenderings/env_ennis/28_37_leather_tiles_4_outputs-rerendering.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/4/images/28_37_leather_tiles_4-outputs_gammad-0-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/4/images/28_37_leather_tiles_4-outputs_gammad-1-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/4/images/28_37_leather_tiles_4-outputs_gammad-2-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/4/images/28_37_leather_tiles_4-outputs_gammad-3-.png} & \vspace{3mm} \\
\begin{sideways} \hspace{-5mm} \small{Ground Truth} \end{sideways} &   & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/slentedRenderings/28_37_leather_tiles_4_4-targets-_relight.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/envRenderings/env_ennis/28_37_leather_tiles_4_targets-rerendering.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/28_37_leather_tiles_4-targets_gammad-0-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/28_37_leather_tiles_4-targets_gammad-1-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/28_37_leather_tiles_4-targets_gammad-2-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/28_37_leather_tiles_4-targets_gammad-3-.png} & \vspace{3mm}

\end{tabular}

\caption{Adding images allows our method to better capture the geometric and reflectance details of this synthetic material.}
\label{fig:synth5improvement}
\end{figure*}

==> figures/classicalOptim/classicalOptimTable.tex <==
\begin{table*}[t]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline 
Input number (our method) & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\ 
\hline 
RMSE & 0.0584 & 0.0568 & 0.0437 & 0.0440 & 0.0410 & 0.0447 & 0.0439 \\ 
\hline 
SSIM & 0.7973 & 0.8396 & 0.8737 & 0.8805 & 0.8930 & 0.8831 & 0.8845 \\ 
\hline 
Input number (classic optimization) & 4 & 16 & 36 & 64 & 100 & 144 & 196 \\ 
\hline 
RMSE & 0.1556 & 0.0749 & 0.0531 & 0.0308 & 0.0225 & 0.0172 & 0.0161 \\ 
\hline 
SSIM & 0.5145 & 0.8280 & 0.8732 & 0.9207 & 0.9228 & 0.9401 & 0.9490 \\ 
\hline 
\end{tabular} 
\caption{Classical optimization method vs our method}
\label{fig:classicalOptim}
\end{table*}


==> figures/real10Improvement/real10Improvement.tex <==
\begin{figure*}[!t]
\begin{tabular} {cccccccc}
  & \vspace{0.5mm} \small{Inputs}  &  \vspace{0.5mm} \small{Renderings} & \vspace{0.5mm} \small{Normal}  & \vspace{0.5mm} \small{Diffuse albedo}  & \vspace{0.5mm} \small{Roughness}  & \vspace{0.5mm} \small{Specular albedo}  &   \\
\begin{sideways} \hspace{-5mm} \small{1 input} \end{sideways} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/kitchenMosaic-inputs-0-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/slentedRenderings/kitchenMosaic_4-outputs-_relight.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/kitchenMosaic-outputs_gammad-0-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/kitchenMosaic-outputs_gammad-1-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/kitchenMosaic-outputs_gammad-2-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/0/images/kitchenMosaic-outputs_gammad-3-.png} & \vspace{3mm} \\
\begin{sideways} \hspace{-5mm} \small{3 inputs} \end{sideways} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/images/kitchenMosaic-inputs-2-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/slentedRenderings/kitchenMosaic_4-outputs-_relight.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/images/kitchenMosaic-outputs_gammad-0-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/images/kitchenMosaic-outputs_gammad-1-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/images/kitchenMosaic-outputs_gammad-2-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/2/images/kitchenMosaic-outputs_gammad-3-.png} & \vspace{3mm} \\
\begin{sideways} \hspace{-5mm} \small{6 inputs} \end{sideways} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/5/images/kitchenMosaic-inputs-5-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/5/slentedRenderings/kitchenMosaic_4-outputs-_relight.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/5/images/kitchenMosaic-outputs_gammad-0-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/5/images/kitchenMosaic-outputs_gammad-1-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/5/images/kitchenMosaic-outputs_gammad-2-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/5/images/kitchenMosaic-outputs_gammad-3-.png} & \vspace{3mm} \\
\begin{sideways} \hspace{-5mm} \small{10 inputs} \end{sideways} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/9/images/kitchenMosaic-inputs-9-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/9/slentedRenderings/kitchenMosaic_4-outputs-_relight.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/9/images/kitchenMosaic-outputs_gammad-0-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/9/images/kitchenMosaic-outputs_gammad-1-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/9/images/kitchenMosaic-outputs_gammad-2-.png} & \includegraphics[align=c, width=0.12\linewidth]{figures/AllImages/2019/9/images/kitchenMosaic-outputs_gammad-3-.png} & \vspace{3mm} \\
 
 & \\ 
  & \\ 
  & \\ 
  & \\ 
  & \\ 
  & \\ 
  &  
 \\
\label{fig:real10Improvement}
\end{tabular}

\caption{Adding images allows our method to better capture the geometric and reflectance details of this real-world material.}
\end{figure*}
